Text Editing by Command

A prevailing paradigm in neural text generation is one-shot generation, where text is produced in a single step. The one-shot setting is inadequate, however, when the constraints the user wishes to impose on the generated text are dynamic, especially when authoring longer documents. We address this limitation with an interactive text generation setting in which the user interacts with the system by issuing commands to edit existing text. To this end, we propose a novel text editing task, and introduce WikiDocEdits, a dataset of single-sentence edits crawled from Wikipedia. We show that our Interactive Editor, a transformer-based model trained on this dataset, outperforms baselines and obtains positive results in both automatic and human evaluations. We present empirical and qualitative analyses of this model's performance.

==> tables/model_output_examples.tex <==
\begin{table}%
\begin{adjustwidth}{-.0in}{-.0in}
    \centering
    \begin{tabular}{p{0.2\linewidth}p{0.7\linewidth}} \toprule
         Comment & Better Newspaper. \\ \cmidrule(r){2-2}
         \multirow[c]{11}{*}{Reference edit} & When news of his death reached Australia in March 1913, several Australian newspapers--including the "Advertiser", the "Western Argus" and the "\textbf{Barrier Miner}"--ran biographies of Belgrave Ninnis, noting his surveying work in the Northern Territory and Arctic exploration. \\ \\
          & When news of his death reached Australia in March 1913, several Australian newspapers--including the "Advertiser", the "Western Argus" and the "\textbf{Sydney Morning Herald}"--ran biographies of Belgrave Ninnis, noting his surveying work in the Northern Territory and Arctic exploration. \\ \cmidrule(r){2-2}
         \multirow[c]{11}{*}{Model edit} & When news of his death reached Australia in March 1913, several Australian newspapers--including the "\textbf{Advertiser}", the "Western Argus" and the "Barrier Miner"--ran biographies of Belgrave Ninnis, noting his surveying work in the Northern Territory and Arctic exploration. \\ \\
          & When news of his depth reached Australia in March 1913, several Australian newspapers--including the "\textbf{Newcastle Morning Herald}", the "Western Argus" and the "Barrier Miner"--ran biographies of Belgrave Ninnis, noting his surverying work in the Northern Territory and Arctic exploration.\\
         \midrule
         Comment & another minor addition \\ \cmidrule(r){2-2}
         \multirow[c]{5}{*}{Reference edit} & They are more frequent than primary brain tumors. \\ \\
          & They are more frequent than primary brain tumors\textbf{, and are mainly a problem in adults, though children may also have secondary tumors.} \\ \cmidrule(r){2-2}
         \multirow[c]{4}{*}{Model edit} & \textbf{They} are more frequent than primary brain tumors. \\ \\
          & \textbf{Secondary brain tumors} are more frequent than primary brain tumors. \\
         \bottomrule
    \end{tabular}
    \caption{Example outputs from the model for two edits from the test data. The edit shown is the top-ranked generation from beam search, excluding the parrot generation if it occurs. The grounding and context are omitted here for brevity.}
    \label{tab:model_out_examples}
\end{adjustwidth}
\end{table}

\begin{table}%
\begin{adjustwidth}{-.0in}{-.0in}
    \centering
    \begin{tabular}{p{0.2\linewidth}p{0.7\linewidth}} \toprule
         Comment & didnt say who fired the canisters \\ \cmidrule(r){2-2}
         \multirow[c]{11}{*}{Reference edit} & When Jordan was six months old, during the time of the Falls Curfew, when many streets were barricaded and there were frequent riots, he almost died from CS gas after canisters \textbf{entered} the family 's home during an army operation.\\ \\
          & When Jordan was six months old, during the time of the Falls Curfew, when many streets were barricaded and there were frequent riots, he almost died from CS gas after \textbf{the British Army fired} canisters \textbf{into} the family 's home during an army operation.\\ \cmidrule(r){2-2}
         \multirow[c]{11}{*}{Model edit} & When Jordan was six months old, during the time of the Falls Curfew, when many streets were barricaded and there were frequent riots, he almost died from CS gas after canisters \textbf{entered} the family 's home during an army operation. \\ \\
          & When Jordan was six months old, during the time of the Falls Curfew, when many streets were barricaded and there were frequent riots, he almost died from CS gas after \textbf{soldiers fired} canisters \textbf{into} the family 's home during an army operation.\\
         \midrule
         Comment & Added more marriage info. \\ \cmidrule(r){2-2}
         \multirow[c]{5}{*}{Reference edit} & Johnson married Group 1 Crew member Manwell Reyes \textbf{in 2011}. \\ \\
          & Johnson married Group 1 Crew member Manwell Reyes in \textbf{on June 11, 2011 in Half Moon Bay, California}. \\ \cmidrule(r){2-2}
         \multirow[c]{4}{*}{Model edit} & Johnson married Group 1 Crew member Manwell Reyes in 2011. \\ \\
          &  Johnson married Group 1 Crew member Manwell Reyes in 2011 \textbf{in a ceremony at Half Moon Bay, California}. \\
         \bottomrule
    \end{tabular}
    \caption{More example outputs from the model.}
    \label{tab:appendix_model_out_examples}
\end{adjustwidth}
\end{table}
